Motion Sensor-based Privacy Attack on Smartphones

In this paper, we build a speech privacy attack that exploits speech reverberations generated from a smartphone's in-built loudspeaker captured via a zero-permission motion sensor (accelerometer). We design our attack Spearphone2, and demonstrate that speech reverberations from inbuilt loudspeakers, at an appropriate loudness, can impact the accelerometer, leaking sensitive information about the speech. In particular, we show that by exploiting the affected accelerometer readings and carefully selecting feature sets along with off-the-shelf machine learning techniques, Spearphone can successfully perform gender classification (accuracy over 90%) and speaker identification (accuracy over 80%) for any audio/video playback on the smartphone. Our results with testing the attack on a voice call and voice assistant response were also encouraging, showcasing the impact of the proposed attack. In addition, we perform speech recognition and speech reconstruction to extract more information about the eavesdropped speech to an extent. Our work brings to light a fundamental design vulnerability in many currently-deployed smartphones, which may put people's speech privacy at risk while using the smartphone in the loudspeaker mode during phone calls, media playback or voice assistant interactions.

==> tex/Comparison.tex <==
\section{Speech Features in Audio vs Vibration domain}
\label{sec:audioVib}
Voice authentication systems rely on spectral features of a speaker's voice to uniquely identify a speaker. \vv\ uses the effect of speech on accelerometer to capture features of a speaker's voice that are unique per user. Since we used machine learning classifier to evaluate the performance of \vv\, we analyze the the features in our feature set that had the most influence in uniquely identify a speaker. We used information gain to rank the features for each of the datasets across the tested phone models and compared which features constantly ranked among top fifteen out of the fifty eight attributes in the feature set.

% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\caption{Top fifteen features using information gain attribute}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Galaxy S6 Voxforge} & \textbf{Galaxy S6 Arctic} & \textbf{Note 4 Voxforge} & \textbf{Note 4 Arctic} & \textbf{LG G3 Voxforge} & \textbf{LG G3 Arctic} \\ \hline
absAreaz                    & totalAbsArea              & absMeanx                 & absAreax               & q2x                     & q2y                   \\ \hline
totalAbsArea                & absAreaZ                  & energyx                  & absMeanx               & absMeanx                & q3y                   \\ \hline
domFreqZ                    & domFreqZ                  & q2x                      & q2x                    & q1x                     & q1y                   \\ \hline
energyZ                     & energyZ                   & q3x                      & q1x                    & q3x                     & absMeany              \\ \hline
domFreqY                    & entropyZ                  & absAreax                 & q3x                    & absAreax                & q2x                   \\ \hline
entropyZ                    & totalSVM                  & absAreay                 & totalAbsArea           & q2y                     & absAreay              \\ \hline
entropyy                    & energyX                   & absMeany                 & energyx                & absMeany                & cvy                   \\ \hline
absAreay                    & domFreqy                  & q3y                      & q2z                    & absAreay                & absMeanx              \\ \hline
entropyx                    & absAreaX                  & q2y                      & absMeanz               & q3y              & domFreqy              \\ \hline
totalSVM                    & entropyY                  & q1x                      & absAreaz               & q1y                     & q3x                   \\ \hline
mcrX                        & domFreqX                  & q1y                      & energyz                & energyy                 & q1x                   \\ \hline
energyY                     & entropyX                  & totalAbsArea             & q1z                    & domFreqX                & absAreaX              \\ \hline
mcry                        & absMeanX                  & energyY                  & minx                   & totalAbsArea            & energyY               \\ \hline
energyx                     & q1x                       & cvY                      & q3z                    & energyX                 & energyX               \\ \hline
absMeanx                    & q2x                       & domfreqY                 & absAreay               & cvX                     & miny                  \\ \hline
\end{tabular}
\end{table*}

==> tex/future.tex <==

\smallskip 
\noindent \textbf{Potential Future Avenues:}
In this work, we implemented a concrete practical instantiation of \vv\
using the smartphone setup allowing us to utilize both the inbuilt speaker
and the embedded motion sensors in the vibration based authentication
scheme. In future work, \vv\ can also be implemented in a loudspeaker setup where a motion
sensor measures the surface vibrations generated due to the playback of the
user's speech for challenge-response authentication set-up in the background setting. We can also modify the implementation of current voice
assistants to include playback of (some part of) user's command for verifying the
authenticity of the user to execute the said command.

Our experiments consisted of speech datasets that are available for public use
and as such are sanitized for linguistic purpose, although still recorded with
low-end devices in realistic settings. While we also created our own dataset
from human volunteers, we believe a more extensive dataset can be built to
further test the effectiveness of \vv. Such a dataset could also include
scenarios close to much more real-world implementation where the user speech is
mixed with various deliberate background noises or the cocktail party problem
where a user's speech needs to be recognized among a mixture of several
legitimate users' voices. These directions can be pursued in future work.

In addition to adding more extensive datasets to further evaluate EchoVib, we
can explore more aspects in our future work to improve the system performance.
Specifically, we can seek more suitable feature sets, beyond MFCC and
time-frequency features we studied, in the vibration domain to better represent
each individual's distinct voice characteristics in this domain. More robust
machine learning methods (e.g., deep learning) can also be built to learn
complex non-linear unique speech vibrational abstractions for dealing with
various practical noisy environments. 


==> tex/model.tex <==
\section{System Design}
\label{sec:model}

%\underline{Our proposed authentication model, \vv. How the idea for this model was extrapolated from previous two sections and the inner mechanisms of this authentication model. Again, a workflow model similar to Section \ref{sec:basics} should be put here.}

In this section, we will outline the design of the proposed authentication
system and describe its working mechanism. As detailed in Section
\ref{sec:speechMotion}, speech vibrations from an audio source have the
capability to travel through the shared medium and affect the motion sensors on
a smartphone. While the effect may be limited due to low sampling rate of the
motion sensors (restricted by operating system), it can still be
unique and utilized for speaker authentication. 

In our authentication model, we propose to utilize the speech characteristics
captured by the motion sensors found on the smartphone to uniquely identify a
user. While the sampling rate of MEMS motion sensors is around 8-10kHz, they
are limited to a much lower sampling rate as per the on-board Operating
Systems, such as Android on the smartphone (for example, approximately 200Hz or lower
by Android). The fundamental frequency of an adult male is between 85-180Hz and
for an adult female, it ranges from 165-255Hz \cite{freqmale,freqfemale} . As
per Nyquist sampling theorem, a device with sampling rate of 200Hz can only
capture frequencies up to 100Hz from a signal. Thus it may not be able to
capture the full range of frequencies present in the speech though due to
harmonic effect, still it may be possible, as our design shows, to capture some part of the missing
frequencies.

\subsection{System Setup}

Our model can be set up in either \crs\ or \vcs\ depending upon the verification system requirements. In a challenge-response authentication protocol, the challenge consists of a pre-determined passphrase asked by the verifier and a valid audio response must have matching spectral features to a verified user's speech characteristics. In contrast to a voice authentication system where the verification is performed on the response obtained from the user (an audio of the user's voice), our authentication system measures the response of motion sensors by playing back the user's response in background via speakers. In our setup, the verifier uses a smartphone equipped with accelerometer and a speaker (or a loudspeaker system, if possible) wherein the accelerometer captures the speech vibrations traveling through the surface of the smartphone from its on-board speaker. 

\vv\ can also use a loudspeaker and an external motion sensor setup (like a smartphone equipped with motion sensors or an external motion sensor chip) where the motion sensor setup is placed on top of the (or attached to) speaker system to allow it to read the vibrations more accurately.
%or on a shared surface with the speaker system to capture the speech effect. 
%This setup is similar to the experimental setup used in \cite{michalevsky2014gyrophone,anandspeechless} that measured the effect of machine-rendered speech on gyroscope and accelerometer embedded on a smartphone.

In a voice command setup, the user issues a command to the device (for example, a smart home assistant) and the device tries to match the speech features of the spoken command in the vibration domain with a stored profile. To be able to do so, the device plays back the user command through its speaker and measures the response of on-board accelerometer during this process. By playing back the user's voice in the foreground, the system is not only authenticating the user, it is also verifying the given command.

\subsection{Workflow}

The workflow of the proposed authentication model is a multi-step procedure as described below:

\begin{enumerate}[leftmargin=*]
\item \textit{Initialization/Training Phase:} During the initialization phase, the user is required to utter multiple phrases/sentences for training the verification model. \vv\ replays the user's voice input either in the background (\crs) or in the foreground (\vcs) and records the accelerometer readings to measure the impact of surface-borne speech vibrations, generated during the playback from the speakers. \vv\ then extracts speech features from the vibration domain (accelerometer readings) and trains a machine learning classifier on the extracted feature set. The details of the speech feature set and the machine learning classifier are described in Section \ref{sec:featureSet} and Section \ref{sec:classifier}.
%The sentences could be a pre-determined sentence repeated multiple times or multiple sentences spoken in succession. 
%On the remote end, the verifier plays the user's response through a smartphone speaker or a loudspeaker setup and records the motion sensor readings in presence of user's voice. The verifier extracts speech features from every instance of the speaker's utterance and trains a machine learning classifier on the extracted feature set. The details of the speech feature set and the machine learning classifier are described in Section \ref{sec:featureSet} and Section \ref{sec:classifier}.

\item \textit{User Credential Input Phase:} In this phase, the user provides a voice input as a response to a posed challenge (\crs) or a command to execute for the device. The voice input from the user is replayed/echoed through the speaker (in background for \crs\ and in foreground for \vcs) while accelerometer is used to record the speech vibrations. In our implementation, \vv\ uses a smartphone since it has both speakers and on-board accelerometer thus requiring less hardware and more mobility at the cost of limited sampling rate for the motion sensor.
%speaks a phrase into the smartphone after establishing a voice call with the verifier. The verifier captures the user's voice and plays it via speakers in presence of motion sensors. If the verifier setup involves a smartphone, the user's voice can be played via smartphone speakers while utilizing the embedded motion sensors to record the effect of speech on those sensors. If the setup consists of a loudspeaker, the verifier can use either a smartphone's motion sensors or explicit motion sensors (mounted on a motherboard) to record the effect of the speech by pacing the smartphone or the motherboard on top of the loudspeaker. The advantage of using smartphone is that it provides mobility to the verifier while usage of a explicit motion sensors may provide higher accuracy as the motion sensor are free to use their true sampling rate (which is restricted for embedded motion sensors on smartphones). 

\item \textit{Feature Extraction and Verification Phase:} The feature extraction phase consists of extracting the required speech features from the recorded accelerometer readings during speech replay. Once extraction is complete, \vv\ attempts to recognize the speaker based on the speech features fed to the classifier algorithm. If the speech is categorized as belonging to one of the trusted users, the verification is complete, and the user is verified otherwise the user is rejected.
\end{enumerate}


\subsection{Candidate Features \& Classification Models}
\label{sec:featureSet}

\subsubsection{Feature Set}
We will now specify the speech feature sets that can potentially be used to uniquely identify a user based on the provided motion sensor readings. Later, in Section \ref{sec:impl}, we will provide a comparison of the two features sets for our classification problem.  

\noindent \textbf{Mel-frequency Cepstrum Coefficient:}
Mel-frequency Cepstrum Coefficients (MFCC) are popular spectral features that are used in speaker identification. The speech signal is expressed on a mel-frequency scale that consists of logarithmic spaced filter modeling the human ear reception of the speech. MFCC features are not affected by changes in the variation of the vocal chords during speech generation hence present a stable speaker characterization basis.

\noindent \textbf{Time and Frequency Domain Feature Set:}
The time and frequency domain features consist of several statistical measurements of the signal over x, y, and z axis. Some of the features are calculated individually for each axis (for example, minimum, maximum, quartile, inter quartile range) while some of them are calculated over all the three axes (for example, total absolute area of the signal and total signal magnitude averaged over time). The frequency domain features consist of energy (sum of magnitude of FFT coefficients), entropy that captures randomness in the signal, and ratio of magnitude of maximum FFT coefficient to sum of magnitude of all FFT coefficients. Using both time and frequency domain features helps us identify temporal characteristics of the signal in addition to its spectral features (insensitive to phase variation) that make it easier to analyze signal properties in a specific frequency band.

\subsubsection{Classification Algorithms}
\label{sec:classifier}
To classify a speaker based on the extracted feature set, several machine learning algorithms exist that can be used for our purpose. Later, in Section \ref{sec:impl}, we will provide a comparison of the two features sets for our classification problem.   

\noindent \textbf{Support Vector Machine:}
It is a binary classifier that uses a hyperplane to divide the input variable space into two categories. The hyperplane is determined during training phase that uses optimization techniques to maximize the separation of input variables into two classes. For a multi-class scenario, several binary support vector machines can be used in conjunction to categorize the input variables. 
%Sequential minimal optimization (SMO) is a popular training algorithm for support vector machines that is provided in Weka \cite{weka} tool.

\noindent \textbf{Regression based Classifiers:}
A logistic regression classifier predicts the outcome of a dependent variable based on one or more independent variables using a logistic function. 
%Simple Logistic classifier is a regression based classifier provided in Weka.

\noindent \textbf{Decision Tree based Classifiers:}
Random tree and Random forest are decision tree based classifiers that tries to predict the outcome of an output variable when supplied with multiple input variables. The tree nodes represent the input variables while the leaf nodes denote the value of the output variable. Decision trees can suffer from overfitting which is corrected in Random forest method.
%\subsubsection{Gaussian Mixture Model}




==> tex/morphingAttack.tex <==
\section{Effectiveness of \vv\ against\\ Voice Synthesis}
\label{sec:vca}
Voice synthesis attack (Section \ref{sec:rationale}), involves converting a \ssp's voice sample into a voice sample closely resembling a \tsp's voice. In our scenario, any entity that desires to use the system is presented with a \crs\  where a correct response is rewarded with authorized access or a \vcs\ where a voice command is executed only when it is deemed to have originated from a verified speaker. The \textit{challenge-response} game can be text-dependent, text-independent or text-prompted. In a text-dependent setting, a pre-determined passphrase needs to be spoken in an authorized user's voice, while in a text-independent scenario, a natural conversation is established that has to be in the authorized user's voice. Text-prompted setting requires the user to read aloud a given phrase, randomly generated by the system, that should match the voiceprint of a legitimate user.

Voice conversion attacks use statistical modeling techniques to build a model of the \tsp's voice pattern that is then used to map \ssp's voice pattern and regenerate speech in \tsp's voice \cite{cmuvoice}. This method requires only 10-20 sentences in a \tsp's voice to convert any given voice sample into the \tsp's voice. This feature makes these attacks very practical and easy to launch. In voice modeling attack, deep learning is used to build an acoustic model of \tsp's voice using few samples containing only a minute of audio and generate any desired sentence in \tsp's voice. Mukhopadhyay et al. showed that voice conversion attacks have a very high success rate against many existing voice authentication services \cite{mukhopadhyay2015all}, hence we test our proposed system, \vv\ to see if it is able to distinguish between an actual legitimate user's voice and a fake legitimate user's voice that was generated using voice conversion or voice modeling.
\begin{table}[]
\centering
\caption{\vv\ Evaluation using Random forest classification against voice conversion attack. Over 90\% morphed voice sample detection rate indicates the resilience of \vv\ against such attacks.}
\label{tab:voiceConv}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{VoxForge Dataset}}             & \multicolumn{2}{c|}{\textbf{CMU Arctic Dataset}}              \\ \hline
\textbf{Devices}                & \textbf{True Positive} & \textbf{False Positive} & \textbf{True Positive} & \textbf{False Positive}  \\ \hline
Samsung Galaxy S6               & 1.000                   & 0.000                   &  0.994                           & 0.006                                \\ \hline
Samsung Note 4                  & 0.907                   & 0.195                    &0.933                             &0.086                                                           \\ \hline
LG G3                           & 0.952                   & 0.073                    & 0.852                            & 0.149                                                      \\ \hline
\end{tabular}}
\end{table}
\subsection{Attack Setup}
\label{sec:attacksetup}

\subsubsection{Festvox Voice Conversion for CMU{\_}Arctic and Voxforge Datasets}
We used Festvox voice conversion technique to create attacked samples for CMU{\_}Arctic and Voxforge datasets. To synthesize the victim's voice, we used Festvox voice conversion technique  \cite{toda2004acoustic}, which produces the synthesized samples by mapping features of a source speaker's voice (i.e., the attacker) to a target speaker's voice (i.e., the victim). Festvox employs acoustic-to-articulatory inversion mapping based on Gaussian Mixture Model that determines the positions of speech articulators of a speaker from the speech. The system then uses a spectral conversion between speakers for transforming the source speaker's voice to a target speaker's voice. This conversion is independent of the phonetic information of the speech. Festvox voice conversion had been used in the past to create voice samples \cite{esorics-2015} that have been used on Voxforge dataset to fool common voice authentication systems. 

To train the Festvox voice conversion tool we used 50 CMU Arctic sentences spoken by both the source and the target speaker. We selected a male speaker from the CMU Arctic dataset as the attacker (bdl speaker), and as the victim, we selected five female and five male speakers from the CMU Arctic dataset, and ten male speakers from the Voxforge dataset. After training the system, we created 100 samples of the target speaker by feeding the source speaker's sample (bdl) to the trained system. 
\vspace{-2mm}
\subsubsection{Lyrebird Voice Modeling for Amazon Turk Dataset}

Voice modeling technology being offered by Lyrebird \cite{lyrebird} and
Google WaveNet \cite{googlewavenet} aims to generate speech samples that
closely resemble human speech and claim to sound more natural than existing
text-to-speech voice generation systems. This technology uses raw audio
characteristics to build an acoustic model for a given person by training on a
set of voice samples collected from that person.  Advanced machine learning
algorithms, such as deep learning, are utilized to train the acoustic model and
this model can produce speech samples that mimic a person's voice that sound
like any desired phrase or sentence \cite{lyrebirdnews} and as such can be
exploited by such an attacker.

To create the synthesized voice for the Amazon Turk dataset, we used the Lyrebird voice synthesis tool. Lyrebird is a recent speech synthesis approach that relies on deep learning techniques to extract features of the speaker's voice from only a few minutes of the speech and produce naturally sounding samples in the speaker's voice. 

Since Lyrebird has not yet officially published their API, we created the samples using Lyrebird web-based voice synthesizers. To collect the data we published a HIT on Amazon Turk and asked the participants to record their voice on Lyrebird website. The participants were compensated \$3 for their effort. The participants were informed that the purpose of this task is to evaluate the performance of a speech synthesis tool. We also informed them that these samples would solely be used for the research. Note that Amazon Turk IDs do not identify the users and therefore the collected audio does not carry any identification parameter. 

We created ten accounts on Lyrebird and asked each of the 10 Turk users to log in to one of these accounts and record their voice as instructed by Lyrebird web-based tool speaking 50 sentences displayed on the website. These recorded samples are used to train the Lyrebird speech synthesizer to create a model of the speaker's voice. Using this model, we generated 100 samples of the speaker's voice using Lyrebird text to speech tool. 

\subsection{\vv\ vs. Voice Conversion Attack}
\label{sec:echoVca}
We will now describe the performance of \vv\ when it is presented with fake voice samples generated by exploiting a legitimate user's voice and observe its ability to distinguish between a legitimate user's voice sample and the fake voice sample generated in the legitimate user's voice by an attacker. We train our random forest classifier on legitimate voice samples of a speaker and then evaluate the true positive and false positive rate of this classifier when presented with fake voice samples of the targeted speaker. A low value of false positive rate would indicate that \vv\ was able to identify most of the fake voice samples as not belonging to the speaker and hence rejects them. This is a desired trait for our speaker authentication system.

As in Section \ref{sec:spkClass}, we use the same datasets (58 samples per speaker for Voxforge, 100 samples per speaker for CMU{\_}Arctic) for training our \vv\ verification model with random forest as the classification algorithm. We show the true positive and false positive rate for detecting fake samples in Table \ref{tab:voiceConv}. The table shows that \vv\ can detect fake samples with a high true positive rate ($>0.900$) for all phone models for Voxforge dataset and CMU{\_}Arctic dataset. Since the fake samples were generated using a technique that has been shown to be successful against voice authentication system \cite{mukhopadhyay2015all}, our results seem to promise a much better success rate in detecting the fake voice samples.


\subsection{\vv\ vs. Voice Modeling Attack}
\label{sec:echoVma}

We tested the Amazon Turk dataset that was created for generating morphed voice samples of users using Lyrebird deep learning technology and test it against \vv. Similar to voice conversion attacks, we train our random forest classifier to identify legitimate user's voice samples and then test the morphed voice samples against the classifier. A high true positive rate for morphed samples would indicate that \vv\ was successful in identifying (and thus rejecting) morphed samples that do not match with any of the stored users' speech vibration pattern.
The results of the experiment are detailed in Table \ref{tab:voiceModel}. We observe that morphed samples were identified correctly with high true positive rate (over 0.850) for all the implementations of \vv. Since, voice modeling techniques aim to reproduce any speech sample from limited voice samples of a user, in a very natural voice, our results show that these tools cannot be exploited to fool \vv\ into accepting an artificially generated voice sample as belonging to a legitimate user.

\begin{table}[]
\centering
\caption{\vv\ Evaluation using Random forest classification against voice modeling attack using Lyrebird. Morphed sample detection rate was over 85\% indicating the resilience of \vv\ against these attacks.}
\label{tab:voiceModel}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{Amazon Turk Dataset}}                        \\ \hline
\textbf{Devices}                & \textbf{True Positive} & \textbf{False Positive}  \\ \hline
%Samsung Galaxy S6               &                    &                              \\ \hline
Samsung Note 4                  & 0.869                   & 0.131                     \\ \hline
LG G3                           & 0.998                   & 0.002                                               \\ \hline
\end{tabular}}
\end{table}
%\begin{table}[]
%\caption{Random forest classification accuracy averaged over 10 speakers against voice conversion attack (Voxforge Dataset) }
%\label{tab:voiceConVoxforge}
%\begin{tabular}{|c|c|c|}
%\hline
%\textbf{Devices}  & \textbf{\begin{tabular}[c]{@{}c@{}}Original vs Morphed \\ Accuracy using 10-fold \\ cross validation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Original (training data) vs\\ Morphed (test data) \\ Accuracy\end{tabular}} \\ \hline
%Samsung Galaxy S6 &                                                                                                                    & \textbf{}                                                                                                      \\ \hline
%Samsung Note 4    &0.890                                                                                                                    &0.425 \textbf{}                                                                                                      \\ \hline
%LG G3             &                               0.939                                                                                     & \textbf{}                                                                                                      \\ \hline
%\end{tabular}
%\end{table}



%\begin{table}[]
%\caption{Random forest classification accuracy averaged over 10 speakers against voice conversion attack  (CMU Arctic Dataset)}
%\label{tab:voiceConCMU}
%\begin{tabular}{|c|c|c|}
%\hline
%\textbf{Devices}  & \textbf{\begin{tabular}[c]{@{}c@{}}Original vs Morphed \\ Accuracy using 10-fold \\ cross validation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Original (training data) vs\\ Morphed (test data) \\ Accuracy\end{tabular}} \\ \hline
%Samsung Galaxy S6 &                                                                                                                    & \textbf{}                                                                                                      \\ \hline
%Samsung Note 4    &     0.922                                                                                                               &0.495 \textbf{}                                                                                                      \\ \hline
%LG G3             &              0.852                                                                                                      & \textbf{}                                                                                                      \\ \hline
%\end{tabular}
%\end{table}


%\subsection{\vv\ vs Voice Synthesis Attack}
%Google wavenet and Lyrebird samples
%\subsubsection{Voxforge Dataset}
%
%\subsubsection{CMU{\_}Arctic Dataset}

==> tex/overview.tex <==
\section{Our Approach}
\label{sec:overview}


We will now provide an overview of our proposed \vv\ authentication system and present the design reasoning that shaped up our development of the proposed system, based on its threat model.


\subsection{Overview}

Traditional voice authentication schemes utilize spectral features of speech to
classify users. In our authentication scheme, we propose to use the effect
of speech on motion sensors (accelerometer, in particular) such as the ones ubiquitously found
in smartphones. The speech, when played via speakers, generates a vibrational
response on the enclosing device (in case of smartphone) or on the encasing
body and surrounding surface (in case of loudspeaker). This vibrational
response is created due to the motion of the speaker cone/diaphragm which in
turn is produced due to an underlying coil motion generated due to varying
magnetic field. Our authentication model assumes that the speech features that
form the basis of voice authentication, also produce a unique response in the
vibration pattern of the speaker diaphragm (henceforth referred to as vibrational
features of speech) that can be recorded by the motion sensors and utilized for
speaker recognition. 

\begin{figure}[th]
    \centering
    \includegraphics[width=\columnwidth, height=4cm]{../fig/UserEchoVib1.pdf}
    \caption{\vv\ high-level design in the benign setting depicting different use cases with foreground and background playback. Our implementation reported in thispaper uses smartphone with its embedded motion sensor (accelerometer) as verifier  in ``voice replay in background'' setup.}
    \label{fig:design}
\end{figure}

\begin{figure}[th]
    \centering
    \includegraphics[width=\columnwidth, height=4cm]{../fig/AttackEchoVib1.pdf}
    \caption{EchoVib threat model showcasing the security of vibration domain compared to audio domain under voice synthesis attacks}
    \label{fig:threat}
\end{figure}
Figure \ref{fig:design} shows a high-level overview of our \vv\ authentication model
depicting a benign use case scenario. The verification
system uses speakers (on smartphone or external loudspeaker system) to play the
speech samples of the user which are then recorded by motion sensors. Both the speakers and the motion sensor are trusted entity and cannot be tampered by an attacker. A
smartphone has inbuilt motion sensors while the verification system will have
to use either an external motion sensor setup sharing a surface with the speaker or embedded motion sensors of a 
smartphone by placing the smartphone on a shared surface. Once the vibrational features of speech have been recorded, they can
be used to uniquely identify a user. 

In the benign use case scenario, the user needs to train \vv\ on their speech
samples similar to voice authentication systems. \vv\ can either play the
speech samples provided by the user in \textit{background} (for example,
delegating the task of replaying the speech via loudspeakers and recording its
effect on motion sensors to a remote service) in a \crs\ or in the
\textit{foreground} (like smart voice assistant or a smartphone that can replay
the user's speech after the user provides their speech sample, as a \vcs). \vv\
builds a speech profile for each user by performing feature extraction and
machine learning on the motion sensor readings recorded during the replay of
the training samples.  Once the training is complete, a user's speech sample
can be tested for verification by replaying the speech sample, recording its
response on motion sensor, and performing feature extraction and classification
of the recorded response against the trained model.

The attack scenario (visualized in Figure \ref{fig:threat}) works similar to the benign use scenario, where we assume
the attacker can access the \vv\ system that secures the user's resources. The
attacker is able to provide a speech sample to \vv\ that replays the provided
speech sample and records its effect on motion sensor. After performing feature
extraction, it either matches the given sample with a stored user profile or
rejects the provided speech samples if no matches are found. Of course, if our system were to 
work well the attacker should be rejected. 

Traditional voice authentication systems that naturally work with the audio signals of the users' speech may suffer from \vsa. In \vsa, the attacker tries
to transform its voice to a similar sounding voice of the victim by manipulating
the spectral features of their speech sample either through voice conversion or
voice modeling. The generated voice samples have similar spectral features as
the victim's voice and hence tend to fool the verification system into
authenticating that the attacker as the actual victim as these systems match
the speech features in only the audio domain.
%Synthesized speech attack involves manipulating the public speech samples of
%the victim into the speech sample that is used by the verification system to
%authenticate the victim. 
In our approach, in contrast, we believe that the vibration features of speech cannot be copied by spectral
mimicking of the speech sample in the audio domain and hence the morphed
samples created by the attacker will not generate the same vibrations as the
actual samples in victim's voice.

%or synthesized to create a new speech sample that has similar vibrational
%feature as the verified speech sample of the victim.  In Section
%\ref{sec:morph}, using morphed samples, we show that 


\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth, height=8cm]{../fig/accelAudioOrig.pdf}
\vspace{-5mm}
\caption{A comparison of speech features in audio domain and vibration domain for two speakers ``ljm" and ``lnh" (CMU{\_} Arctic dataset) speaking the following sentence ``You, you would not keep the truth from me.''}
\label{fig:accelAudioOrig}
\end{figure*}

\begin{figure*}[]
\centering
\includegraphics[width=0.9\textwidth, height=8cm]{../fig/accelAudio.pdf}
\vspace{-5mm}
\caption{A comparison of speech features in audio domain and vibration domain for original speaker ``ljm" and her synthesized speech generated using Festvox Transform voice conversion (CMU{\_} Arctic dataset) speaking the sentence ``You, you would not keep the truth from me.''}
\label{fig:accelAudio}
\end{figure*}
\subsection{Design Rationale}
\label{sec:rationale}

\noindent
\textbf{Benign Setting:} 
The underlying fundamental principle behind \vv\ is the uniqueness of the
speech pattern in vibration domain as recorded by the motion sensors. In
traditional voice authentication systems, speech features are extracted from a
recording of a legitimate user's speech to build a speech profile for that
user. We term this process as \textit{speech pattern in the audio domain} as the
speech features are extracted from the audio recording of the speech. In
contrast, our proposed system \vv\ uses the effect of speech on motion sensors
and extracts features from this recording of motion sensor readings in presence
of speech to build a user's profile, hence termed as \textit{speech pattern in
the vibration domain}.




Figure \ref{fig:accelAudioOrig} shows the effect of audio on accelerometer when
the system plays back a speaker's voice sample while recording accelerometer
readings. In the figure, we present two audio samples, one recorded for speaker
``ljm'' and other for speaker ``lnh'' taken from the CMU{\_}Arctic dataset
\cite{arctic} speaking the same sentence ``You, you would not keep the truth
from me''. In the audio domain, we can see noticeable difference between the
speech pattern of the two speakers, especially for each individual word. For
example, the first word ``You'' (denoted by the first yellow band of energy on
the spectrum) is wider for speaker ``ljm'' when compared to speaker ``lnh''.
This pattern is also reflected in the vibration domain as we can see a narrow
column of energy (around $t=1sec$) for speaker ``lnh'' while it is wider and
diffused for speaker ``ljm''. Thus, we believe that uniqueness of speech
pattern among different speakers is retained in the vibration domain as well.


%one in the original voice of the user and the other in a morphed voice (generated from the user's voice sample as discussed in Section \ref{sec:vca}) as created by an attacker using voice conversion techniques.
\noindent
\textbf{Threat Model and Attack Setting:} Audio domain voice authentication has been shown to be susceptible to multiple attack vectors that aim to gain unauthorized access by presenting the authentication system, a speech sample closely resembling a legitimate user's voice. In this work, we consider two such types of attacks namely voice conversion attack and voice modeling attack. We do not consider voice replay attacks in our threat model as naive implementation of such attacks pose limited security threat. A word by word replay of the user's voice commands in either a \crs\ or a \vcs\ would not have a critical security impact unless the attacker manages to synthesize the recording to have a different intent than the original command.

\label{sec:threat}

Our attack model can be defined by three phases: audio sample collection, voice synthesis model generation, and attacking voice authentication systems using synthesized voice samples. In the first phase of \textit{audio sample collection}, the attacker aims to collect sufficient speech samples in a targeted victim's voice. This task can be performed by eavesdropping and recording the victim's voice unknown to them using a hidden voice recorder, or by collecting publicaly available speech samples in victim's voice (through videos hosted on popular social media platforms). In the second phase of the attack \textit{voice synthesis model generation}, the attacker attempts to build a voice synthesizing system that is trained on the collected voice samples of the victim in the first phase. The model takes in a speech sample (not in the victim's voice) and generates a speech sample that closely resembles the speech pattern of the victim.

Once the attacker has trained the voice synthesis system on an intended victim's speech samples, it can try to gain unauthorized access to sensitive information or resources that are confidential to the victim and secured via a voice authentication mechanism. For this purpose, we also assume that the attacker has temporary or permanent access to victim's device that is normally used by the victim and holds the sensitive information or resources. The attacker can then play the synthesized voice sample to the device and tries to get authenticated by the voice authentication system for nefarious purpose. In another scenario, the attacker can try to fool a remote voice authentication system (such as online banking etc.) by playing responses crafted by the voice synthesizing system in victim's voice and attempts to exploit the victim by illegally gaining access to victim's confidential data and resources (for example, bank account details, passwords, PINs etc.).
%
%The proposed authentication system \vv\ is also aimed at providing security against voice conversion attacks. It has been shown that such attacks can deploy voice morphing models, trained on samples of an intended victim's speech samples, and generate morphed speech closely resembling the victim's speech pattern. 
Figure \ref{fig:accelAudio} shows a comparison of original speech and attacker-generated speech for a speaker in audio and vibration domain. In audio domain, the power spectrum for both speech samples show similar pattern though the morphed speech has more diffused spread of energy compared to the original sample. However their effect in vibration domain is not the same especially differing in concentration of power (denoted by yellow) over the frequency range. Thus, we believe that vibration domain is helpful in capturing spectral features that cannot be imitated by the morphing model of the attacker.




==> tex/summaryDiss.tex <==
\section{Discussion and Future Work}



\noindent \textbf{Summary of Results:} Our results for the proposed \vv\ speaker authentication system  show that it is very efficient at performing multi-speaker and binary speaker classification. \vv\ was tested on multiple datasets utilizing different devices that housed different hardware, and \vv\ delivered a consistent accuracy across each tested scenario. We used smartphones in our experiments to implement a basic concept of \vv\ and its effectiveness shows that the proposed scheme is practical as it can be implemented on devices housing motion sensors with low sampling rate. Thus, the effectiveness would increase in a setup with more sophisticated motion sensors even if used in an increasingly noisy environment. Since Anand et al \cite{anandspeechless} showed that it may not be possible for live human voice to affect inbuilt motion sensors, our proposed method would work even in a noisy environment that may affect the usability of voice authentication systems that exist solely in audio domain.

\vv\ was also tested against \vsa\ such as the voice conversion attack and the voice modeling attack. Our results indicated that \vv\ was effective at identifying and rejecting the synthesized voice samples that were generated to imitate a verified user's voice by an attacker. Since voice synthesis attacks can fool many state-of-the-art voice authentication systems, our proposed system provides a viable alternative that is easy to implement either as a stand-alone system or alongside an existing voice authentication system (two-factor/multi-factor authentication).

\smallskip
\noindent \textbf{Limited Sampling Rate and Sensor Fusion:} Limited sampling rate of motion sensors on smartphones was a challenge in the design of \vv\ as it relies on sensitiveness of the motion sensor to speech vibrations generated via speakers. However, our experiments have shown that even in this limited capability, speech footprints recorded in vibration domain have unique features that allow for an accurate speaker classification. We expect the performance of \vv\ to improve in a more natural environment if more sophisticated motion sensors are utilized for authentication in vibration domain. In addition, multiple sensors can possibly be used by interleaving their data output so as to artificially increasing the combined sampling rate, overcoming the imposed restriction from the Operating System.

\smallskip
\noindent \textbf{Foreground vs. Background Playback: }\vv\ design allows for both foreground and background playback of user's voice input. While the background playback maybe a preferred scenario for a \crs, foreground playback of user's input introduces a sense of transparency in \vcs\ especially in the light of some recent attacks that aim to introduce malicious voice commands hidden in inconspicuous audio signals \cite{carlini2016hiddenvoice}. \vv\ allows the user to verify themselves as well as the voice command that was issued, thereby increasing the transparency and convenience of the overall system.

\smallskip
\noindent \textbf{\vv\ for Two-factor Authentication:}
In our implementation of \vv, we tested it as a stand-alone verification system where the speaker's identity was solely determined based on the speech vibration features as recorded by an accelerometer in vibration domain. \vv\ can also be used alongside traditional voice-based authentication system wherein a speaker would be verified in both audio domain and vibration domain. A user will be granted access if it matches the profile of a legitimate user in both the domains. Such a system would be resilient to voice synthesis attacks as these attacks have been shown to be ineffective against \vv. Since \vv\ only hardware requirement is a speaker and motion sensor, it can practically be implemented alongside any system. For \crs\ like remote caller verification in online financial service, background playback feature of \vv\ can be utilized where the task of recording the speech vibration is offloaded to a trusted third-party cloud service that is equipped with required hardware. In \vcs, most of smart device already come equipped with speakers and may only require an on-board motion sensor (similar to a smartphone hardware design).

%\subsection{Multiple Device Training}
\smallskip
\noindent \textbf{Potential Sophisticated Vibration Morphing Attack:} Speech vibrations in the vibration domain form the backbone of our proposed authentication model. A possible attack vector could be created by attempting to generate vibrations that mimic the speech vibrations of a legitimate user. In this attack, the attacker may recreate a possible playback scenario (as used in \vv) and record motion sensor readings by replaying a previously eavesdropped voice sample of the user. The attacker can then try to fool \vv\ by imitating the vibration pattern recorded earlier by the attacker that matches with  the user's speech vibrations. However, this attack vector will pose significant challenges in practice. First of all, for the challenge-response authentication systems, replay attacks would not really work. Second, the challenge-response voice authentication systems and voice assistant systems already deploy a speech-to-text transcriber to learn the response/command from the user, which means that the attacker would have to create a transcribable audio signal in addition to matching the vibrational features, a difficult task in practice. 

==> tex/verificationExp.tex <==
\section{Implementation and Evaluation}
\label{sec:impl}

In this section, we report on the implementation of an instance of the proposed \vv\ authentication system as per the system design detailed in Section \ref{sec:model}. We also present the evaluation of our implementation in the benign setting. 

\subsection{Setup and Preliminaries}
\label{sec:setup}
\noindent \textbf{Voice Datasets: } 
To test \vv, we used Voxforge dataset \cite{voxforge}, CMU{\_}Arctic dataset \cite{arctic}, and a speech dataset built using Amazon Turk workers. For Voxforge and CMU{\_}Arctic datasets, we selected ten speakers reading CMU{\_}Arctic sentences. We use CMU{\_}Arctic dataset as it provides over 100 samples per speaker while Voxforge dataset was chosen especially for testing voice conversion attacks as it has been shown susceptible to these attacks \cite{mukhopadhyay2015all}. ``Amazon Turk dataset'' was created for testing Lyrebird speech modeling attack that uses Lyrebird web-based audio recording tool. To build this dataset, we published an IRB approved Amazon Turk HIT and asked ten workers (American English accent) to speak and record sentences provided by Lyrebird web-based tool. Participation in the survey
was voluntary and the participants could withdraw any time. We converted all samples to WAV file format at 16 kHz sampling rate. The spoken sentences in all of our datasets were short in length averaging about 8 words per sentence.
%We considered two open source speech datasets, namely CMU{\_}Arctic dataset \cite{arctic} and Voxforge dataset \cite{voxforge} for our speaker. For each of these datasets, we selected ten speakers reading CMU{\_}Arctic sentences. We also built a third dataset specifically for Lyrebird speech synthesis tool using Lyrebird web-based audio recording tool. We refer to this dataset as ``Lyrebird dataset''. To build this dataset, we published an IRB approved Amazon Turk HIT and asked ten workers (American English accent) to speak and record sentences provided by Lyrebird web-based tool. We converted all samples to WAV files at 16 kHz sampling rate. More details on these datasets is provided in Section \ref{sec:attacksetup}.

\medskip
\noindent \textbf{Equipment: } While \vv\ is designed to be used with any speaker (loudspeaker or inbuilt device speaker) and motion sensors (external motion sensors or on-board motion sensor on the device), we have used smartphone as the device to implement \vv. A smartphone houses both a speaker and on-board motion sensors on the same device, providing a convenient setup for \vv. We used three different smartphones Samsung Galaxy S6, Samsung Note 4, and LG G3 to act as devices to implement \vv.

Samsung Galaxy S6 and LG G3 have Invensense MPU-6500 as the embedded motion sensor chip housing a 6-axis gyroscope and accelerometer. Samsung Galaxy Note 4 has Invensense MPU-6515 as the motion sensor chip that has similar capability as MPU-6500. These motion sensor chips have similar output data rates to other embedded motion sensors on smartphones available in the market, that is restricted by Android platform to be around 200Hz. In addition, they share similar physical characteristics such as mechanical resonant frequency and precision with other popular phones in the market. Hence, we believe our choice of phones represents a fair variety of motion sensor capabilities.

On each smartphone, we install a custom sensor logging application developed on Android platform that records motion sensor readings, while response from the user is being played on the speakers of the phone. The phone was kept flat on a wooden surface with no external motion being present in the surrounding environment. Another possible scenario involves keeping the phone hand-held where it may be in motion due to user's body movement. In case of a user walking while holding the phone, it has been observed \cite{zhang2015accelword} that the effect of such motion can be eliminated by applying a high pass filter ($> 2$Hz) on the recorded signal.

\medskip
\noindent \textbf{Signal Processing and Machine Learning Tools: } Once the sensor readings were recorded by our application, we transferred the log file containing the readings to an offline system for processing. In real world, \vv\ can send the sensor readings to a trusted cloud server that processes them for verification and returns the result to \vv. It could also be implemented on the device itself provided the device contain enough processing resources and there exists no power constraint. For processing the sensor readings, we used Matlab's signal processing functions to extract the relevant feature set from each recorded sample. The classification model was trained and tested on Weka toolkit \cite{weka} that provides a workbench for implementing various machine learning algorithms.


%\subsection{Classifier and Feature Set Selection}
%For choosing the most accurate classifier and the best feature set for our proposed authentication system \vv,  we  perform an initial experiment on the Voxforge dataset to compare multiple classifiers (described in Section \ref{sec:classifier}) on different feature sets (as described in Section \ref{sec:featureSet}). In particular, we tested both MFCC features and Time-frequency domain feature set to classify our recorded samples. 
%%MFCC feature set was used by Michalevsky et al. \cite{michalevsky2014gyrophone} for gender and speaker classification on TIDigit dataset from gyroscope readings from a smartphone while time-frequency domain feature set was used by Zhang et al. \cite{zhang2015accelword} to detect and classify hotwords on a smartphone using accelerometer readings.
%We used support vector machine, decision trees and regression based classifiers to assess their performance on both feature sets and chose the classifier that was most efficient in speaker classification (based on the performance metrics detailed in Section \ref{sec:metrics}).
%For machine learning classifiers, support vector machines were used by Michalevsky et al. \cite{michalevsky2014gyrophone} while decision trees were used by Zhang et al. \cite{zhang2015accelword} for their classification purpose. We tested both classes of machine learning algorithms along with a regression based classifier, Simple Logistic classifier to complete our analysis. 

%\medskip
%\noindent \textbf{Results:}
%The results from our analysis on the Voxforge dataset using the three phone models are detailed in Table \ref{tab:accelVox} and \ref{tab:mfccVox}. Using the metrics described in \ref{sec:metrics}, we observe that time-frequency domain features performed better than MFCC feature set with an f-measure value $>0.900$ for all three phone models compared to MFCC feature set that showed a best f-measure value of $0.752$ for Samsung Note 4 and $0.845$ for LG G3. For classification, random forest classifier outperformed other classifiers with an f-measure value $> 0.900$ for all three phone models compared to other classifiers (f-measure value slightly below $0.900$). Thus, we choose time-frequency domain feature set and random forest classifier to implement \vv\ for the rest of our work.


\medskip
\noindent \textbf{Classification Metrics:}
\label{sec:metrics}
We use the following metrics to determine the classifier accuracy for speaker recognition.

\smallskip
\noindent\textit{Precision:} It is defined as the ratio of correct class predictions to total number of classes.

\begin{equation}
Precision = \frac{true~positive}{true~positive + false~positive}
\end{equation}

\smallskip
\noindent\textit{Recall:} It is defined as the ratio of correct class predictions to total number of correct class instances.
\begin{equation}
Recall = \frac{true~positive}{true~positive + false~negative}
\end{equation}

\smallskip
\noindent\textit{F-measure:} It is the harmonic mean of \textit{precision} and \textit{recall} attaching equal weights to both precision and recall values.

\begin{equation}
F\textnormal{-} measure = \frac{2 \times precision \times recall}{precision + recall}
\end{equation}

\subsection{Comparing Feature Sets and Classifiers}

\begin{table*}[th]
\centering
\caption{10 speaker classification using time-frequency features on Voxforge dataset (10-fold cross validation). Random Forest provides the highest accuracies.}
\label{tab:accelVox}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Phone Model}         & \multicolumn{3}{c|}{\textit{\textbf{Samsung Galaxy S6}}}  & \multicolumn{3}{c|}{\textit{\textbf{Samsung Note 4}}}     & \multicolumn{3}{c|}{\textit{\textbf{LG G3}}}              \\ \hline
\textbf{Classifiers}         & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} \\ \hline
Simple Logistic              & 0.871              & 0.841           & 0.850              &0.878                    &0.877                 &0.877                    &  0.941                  &    0.940             &     0.940               \\ \hline
Support Vector Machine (SMO) & 0.887              & 0.881           & 0.880              &0.894                    &0.890                 &0.890                    & \textbf{0.946}                  &     \textbf{0.945}            &   \textbf{0.945}                 \\ \hline
Random Forest                &\textbf{0.959}              & \textbf{0.959}           & \textbf{0.999}              &\textbf{0.907}                    &\textbf{0.907}                 &\textbf{0.906}                    &    0.941                &    0.939            &     0.939               \\ \hline
Random Tree                  & 0.873              & 0.871           & 0.928              &0.790                    &0.788                 &0.788                    &     0.917               &    0.916             &    0.916                \\ \hline
J48 Tree                     & 0.886              & 0.884           & 0.949              &0.827                    &0.827                 &0.825                    &    0.924                &    0.922             &    0.922                \\ \hline
\end{tabular}}
\end{table*}

\begin{table*}[]
\caption{10 speaker classification using MFCC features on Voxforge dataset (10-fold cross validation). Random Forest provides the highest accuracies.}
\label{tab:mfccVox}
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Phone Model $\rightarrow$}         & \multicolumn{3}{c|}{\textit{\textbf{Samsung Galaxy S6}}}  & \multicolumn{3}{c|}{\textit{\textbf{Samsung Note 4}}}     & \multicolumn{3}{c|}{\textit{\textbf{LG G3}}}              \\ \hline
\textbf{Classifiers $\downarrow$}         & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} \\ \hline
Simple Logistic              & 0.796              & 0.740           & 0.754              & 0.729                   &        0.728         &     0.727               &    0.846                &    \textbf{0.845}             &      \textbf{0.845}              \\ \hline
Support Vector Machine (SMO) & 0.872              & 0.871           & 0.869              &         0.686           &      0.685           &      0.685              &   0.801                &    0.800             &     0.800               \\ \hline
Random Forest                & \textbf{0.913}              & \textbf{0.912}           & \textbf{0.912}              &    \textbf{0.753}                &      \textbf{0.753}           &     \textbf{0.752}               &   \textbf{0.846}                 &    0.844             &    0.844                \\ \hline
Random Tree                  & 0.771              & 0.767           & 0.767              &     0.580               &      0.580           &        0.580            &        0.687            &    0.686             &    0.686                \\ \hline
J48 Tree                     & 0.837              & 0.836           & 0.836              &    0.728                &        0.727         &       0.726             &           0.820         &      0.819           &    0.819                \\ \hline
\end{tabular}}
\end{table*}



While both MFCC features and time-frequency domain features can be used to
classify a speaker's voice in \textit{audio domain}, our implementation
requires a feature set that works well in the \textit{vibration domain}. We
compared the accuracy of both the feature sets using the classifiers discussed
in Section \ref{sec:classifier} and the metrics stated in Section
\ref{sec:metrics}. We tested three smartphones, multiple datasets and signal
processing tools as described in Section \ref{sec:setup}.

The results from our feature set comparison study on the Voxforge dataset are
detailed in Table \ref{tab:accelVox} and \ref{tab:mfccVox}. Using the metrics
described in \ref{sec:metrics}, we observe that time-frequency domain features
performed better than MFCC feature set with an f-measure value $>0.900$ for all
three phone models compared to MFCC feature set that showed the best f-measure
value of $0.752$ for Samsung Note 4 and $0.845$ for LG G3. For classification,
random forest classifier outperformed other classifiers with an f-measure value
$> 0.900$ for all three phone models compared to other classifiers (f-measure
value slightly below $0.900$).  Hence, in the rest of our evaluation, we proceed 
with Random Forest along with the time-frequency domain feature set.  

MFCC features are more suitable for audio signals that are sampled at a higher
frequency than motion sensor's sampling rate that is restricted to
approximately 200Hz by the Android platform in our setup. Thus, we believe
time-frequency domain feature set captures more information about the speech
vibration than MFCC feature set leading to a better speaker classification
accuracy. Thus, we choose time-frequency domain feature set and random forest
classifier to implement \vv\ for the rest of our work.

This initial result also confirms the premise of \vv\ that relies on
measurement of speech impact on motion sensors in vibration domain. Motion
sensors, due to their limited sampling rate, may not be deemed capable of
capturing audio features that are better captured by a microphone. However, the
measured vibrations by these motion sensors can be deemed unique as shown by
our results here and on the power spectrum in Figure \ref{fig:accelAudioOrig}.

%Also these results indicate that Random Forest is the classification model providing the 
%highest classification accuracies. 


\subsection{Speaker Classification}
\label{sec:spkClass}
We used 58 voice samples each from 10 speakers belonging to the Voxforge dataset, 100 samples each from 10 speakers belonging to the CMU{\_}Arctic dataset, and 50 samples from each of the 10 speakers in Amazon Turk dataset. Since the samples in these datasets consist of complete sentences, we use the entirety of the recorded sensor reading for the voice sample to extract relevant speech features from the sensor readings. We used Galaxy S6, Note 4 and LG G3 for Voxforge and CMU{\_}Arctic datasets, and Note 4 and LG G3 for Amazon Turk dataset.

\subsubsection{10-Speaker Multiclass Classification}
10-speaker classification involves a multiclass classifier labeling the test samples as one of the ten predefined speakers in each of our datasets. It identifies a speaker's voice among a collection of multi-speaker dataset. An example for 10-speaker classification can be a use case scenario involving a smart home device used by a family where in the inbuilt smart voice assistant answers an individual's query based on that family member's stored profile. 

Our results from 10-speaker classification using 10-fold cross-validation method and random forest classifier are shown in Table \ref{tab:spkClassVox} for Voxforge dataset, Table \ref{tab:spkClassArctic} for the CMU{\_}Arctic dataset, and Table \ref{tab:spkClassLyre} for ``Amazon Turk dataset''. For Voxforge dataset, \vv\ had the most accurate speaker classification with an f-measure value of over 0.999. CMU{\_}Arctic dataset also provided a highly efficient f-measure score (around 0.909) for \vv\ implementation with LG G3 slightly outperforming other phone models.
\begin{table}[h]
\centering
\caption{Speaker classification using 10-fold cross validation and Random Forest classifier (Voxforge Dataset)}
\label{tab:spkClassVox}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|}
\cline{2-4}
                                        & \multicolumn{3}{c|}{\textit{\textbf{10-Speaker Classification}}}    \\ \hline
\multicolumn{1}{|c|}{\textbf{Devices}}  & \textbf{Precision}       & \textbf{Recall}       & \textbf{F-measure}       \\ \hline
\multicolumn{1}{|c|}{Samsung Galaxy S6} & \textbf{0.959}                    & \textbf{0.959}                 & \textbf{0.999}                    \\ \hline
\multicolumn{1}{|c|}{Samsung Note 4}    &0.907                          &0.907                       &0.906                          \\ \hline
\multicolumn{1}{|c|}{LG G3}             &        0.913                  &       0.912                &      0.912                    \\ \hline
                                        & \multicolumn{3}{c|}{\textit{\textbf{One vs Others Speaker Classification}}} \\ \hline
\multicolumn{1}{|c|}{Samsung Galaxy S6} & \textbf{0.986}                    & \textbf{0.986}                 & \textbf{0.985}                    \\ \hline
\multicolumn{1}{|c|}{Samsung Note 4}    &0.978                          &0.980                       &0.979                          \\ \hline
\multicolumn{1}{|c|}{LG G3}             &0.977                          &0.977                       & 0.977                         \\ \hline
\end{tabular}}
\end{table}
\subsubsection{``One vs Others'' Binary Classification}
\begin{table}[]
\centering
\caption{Speaker classification using 10-fold cross validation and Random Forest classifier (CMU{\_} Arctic Dataset)}
\label{tab:spkClassArctic}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|}
\cline{2-4}
                                        & \multicolumn{3}{c|}{\textit{\textbf{10-Speaker Classification}}}    \\ \hline
\multicolumn{1}{|c|}{\textbf{Devices}}  & \textbf{Precision}       & \textbf{Recall}       & \textbf{F-measure}       \\ \hline
\multicolumn{1}{|c|}{Samsung Galaxy S6} &   0.907                  & 0.907                 & 0.906                    \\ \hline
\multicolumn{1}{|c|}{Samsung Note 4}    &      0.909                    &0.908                       &0.908                          \\ \hline
\multicolumn{1}{|c|}{LG G3}             &        \textbf{0.909}                  &       \textbf{0.909}                &      \textbf{0.909}                    \\ \hline
                                        & \multicolumn{3}{c|}{\textit{\textbf{One vs Others Speaker Classification}}} \\ \hline
\multicolumn{1}{|c|}{Samsung Galaxy S6} & \textbf{0.988}                    & \textbf{0.988}                 & \textbf{0.988}                    \\ \hline
\multicolumn{1}{|c|}{Samsung Note 4}    &0.980                          &0.980                       &0.980                          \\ \hline
\multicolumn{1}{|c|}{LG G3}             &0.979                          &0.979                       &0.978                          \\ \hline
\end{tabular}}
\end{table}
``One vs Others'' classification uses a binary classifier to either label a given test samples as belonging to a particular speaker or not. ``One vs Others'' classification scenario regularly occurs on more personal, non-shared devices such as personal phones that are geared to respond only to voice commands of a single authorized entity.

From Table \ref{tab:spkClassVox} and Table \ref{tab:spkClassArctic}, we observe that \vv\ on Galaxy S6 has slightly better accuracy than other tested phone models with a highly efficient f-measure score of 0.985 on Voxforge dataset. For CMU{\_}Arctic dataset, Galaxy S6 implementation of \vv\ outperformed with an f-measure score of 0.988.


%We performed 10-speaker classification and ``One vs Others'' classification for our datasets. 10-speaker classification involves a multi-class classifier labeling the test samples as belonging to one of the ten predefined speakers whereas ``One vs Others'' classification uses a binary classifier to either label a given test samples as belonging to a particular speaker or not. 
%
%10-speaker classification helps in identifying each speaker's voice among a collection of multispeaker dataset while "One vs Others" classification can be considered as a single speaker verification mechanism. An example for 10-speaker classification can be a use case scenario involving a smart home device used by a family where in the inbuilt smart voice assistant answers an individual's query based on that family member's stored profile. ``One vs Others'' classification scenario regularly occurs on more personal, non-shared devices such as personal phones that are geared to respond only to voice commands of a single authorized entity.

%\medskip
%\noindent \textbf{Results:} Our results from 10-speaker classification and ``One vs Others'' classification using 10-fold cross validation method and random forest classifier is shown in Table \ref{tab:spkClassVox} for Voxforge dataset and Table \ref{tab:spkClassArctic} for the CMU{\_}Arctic dataset. The f-measure values ($>$0.90) indicate that the system is reliable in predicting correct speaker in a multi-speaker scenario as well as ``One vs Others'' speaker classification scenario.
\begin{table}[]
\vspace{-2mm}
\centering
\caption{Speaker classification using 10-fold cross validation and Random Forest classifier (Amazon Turk Dataset)}
\label{tab:spkClassLyre}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|}
\cline{2-4}
                                        & \multicolumn{3}{c|}{\textit{\textbf{10-Speaker Classification}}}    \\ \hline
\multicolumn{1}{|c|}{\textbf{Devices}}  & \textbf{Precision}       & \textbf{Recall}       & \textbf{F-measure}       \\ \hline
%\multicolumn{1}{|c|}{Samsung Galaxy S6} &   0                  & 0                 & 0                    \\ \hline
\multicolumn{1}{|c|}{Samsung Note 4}    &      0.949                    &0.949                      &0.949                          \\ \hline
\multicolumn{1}{|c|}{LG G3}             &        0.989                  &       0.989                &      0.989                    \\ \hline
                                        & \multicolumn{3}{c|}{\textit{\textbf{One vs Others Speaker Classification}}} \\ \hline
%\multicolumn{1}{|c|}{Samsung Galaxy S6} & 0                    & 0                 & 0                    \\ \hline
\multicolumn{1}{|c|}{Samsung Note 4}    &0.988                          &0.988                       &0.988                          \\ \hline
\multicolumn{1}{|c|}{LG G3}             &0.997                          &0.997                       &0.997                          \\ \hline
\end{tabular}}
\end{table}

